A star-forming dwarf galaxy candidate in the halo of NGC 4634

The halos of disk galaxies form a crucial connection between the galaxy disk and the intergalactic medium. Massive stars, HII regions, or dwarf galaxies located in the halos of galaxies are potential tracers of recent accretion and/or outflows of gas, and are additional contributors to the photon field and the gas phase metallicity. We investigate the nature and origin of a star-forming dwarf galaxy candidate located in the halo of the edge-on Virgo galaxy NGC 4634 with a projected distance of 1.4 kpc and a H$\alpha$ star formation rate of $\sim 4.7 \times 10^{-3} \text{M}_\odot \text{yr}^{-1}$ in order to increase our understanding of these disk-halo processes. With optical long-slit spectra we measured fluxes of optical nebula emission lines to derive the oxygen abundance 12 + log(O/H) of an HII region in the disk of NGC 4634 and in the star-forming dwarf galaxy candidate. Abundances derived from optical long-slit data and from Hubble Space Telescope (HST) r-band data, H$\alpha$ data, Giant Metrewave Radio Telescope (GMRT) HI data, and photometry of SDSS and GALEX data were used for further analysis. With additional probes of the luminosity-metallicity relation in the $B$-band from the H$\alpha$-luminosity, the HI map, and the relative velocities, we are able to constrain a possible origin of the dwarf galaxy candidate. The high oxygen abundance (12 + log(O/H) $\approx$ 8.72) of the dwarf galaxy candidate leads to the conclusion that it was formed from pre-enriched material. Analysis of auxiliary data shows that the dwarf galaxy candidate is composed of material originating from NGC 4634. We cannot determine whether this material has been ejected tidally or through other processes, which makes the system highly interesting for follow up observations.

==> BIBdef.tex <==
\newcommand{\aj}{AJ}% 
          % Astronomical Journal 
\newcommand{\araa}{ARA\&A}% 
          % Annual Review of Astron and Astrophys 
\newcommand{\apj}{ApJ}% 
          % Astrophysical Journal 
\newcommand{\apjl}{ApJ}% 
          % Astrophysical Journal, Letters 
\newcommand{\apjs}{ApJS}% 
          % Astrophysical Journal, Supplement 
\newcommand{\ao}{Appl.~Opt.}% 
          % Applied Optics 
\newcommand{\apss}{Ap\&SS}% 
          % Astrophysics and Space Science 
\newcommand{\aap}{A\&A}% 
          % Astronomy and Astrophysics 
\newcommand{\aapr}{A\&A~Rev.}% 
          % Astronomy and Astrophysics Reviews 
\newcommand{\aaps}{A\&AS}% 
          % Astronomy and Astrophysics, Supplement 
\newcommand{\azh}{AZh}% 
          % Astronomicheskii Zhurnal 
\newcommand{\baas}{BAAS}% 
          % Bulletin of the AAS 
\newcommand{\jrasc}{JRASC}% 
          % Journal of the RAS of Canada 
\newcommand{\memras}{MmRAS}% 
          % Memoirs of the RAS 
\newcommand{\mnras}{MNRAS}% 
          % Monthly Notices of the RAS 
\newcommand{\pra}{Phys.~Rev.~A}% 
          % Physical Review A: General Physics 
\newcommand{\prb}{Phys.~Rev.~B}% 
          % Physical Review B: Solid State 
\newcommand{\prc}{Phys.~Rev.~C}% 
          % Physical Review C 
\newcommand{\prd}{Phys.~Rev.~D}% 
          % Physical Review D 
\newcommand{\pre}{Phys.~Rev.~E}% 
          % Physical Review E 
\newcommand{\prl}{Phys.~Rev.~Lett.}% 
          % Physical Review Letters 
\newcommand{\pasp}{PASP}% 
          % Publications of the ASP 
\newcommand{\pasj}{PASJ}% 
          % Publications of the ASJ 
\newcommand{\qjras}{QJRAS}% 
          % Quarterly Journal of the RAS 
\newcommand{\skytel}{S\&T}% 
          % Sky and Telescope 
\newcommand{\solphys}{Sol.~Phys.}% 
          % Solar Physics 
\newcommand{\sovast}{Soviet~Ast.}% 
          % Soviet Astronomy 
\newcommand{\ssr}{Space~Sci.~Rev.}% 
          % Space Science Reviews 
\newcommand{\zap}{ZAp}% 
          % Zeitschrift fuer Astrophysik 
\newcommand{\nat}{Nature}% 
          % Nature 
\newcommand{\iaucirc}{IAU~Circ.}% 
          % IAU Cirulars 
\newcommand{\aplett}{Astrophys.~Lett.}% 
          % Astrophysics Letters 
\newcommand{\apspr}{Astrophys.~Space~Phys.~Res.}% 
          % Astrophysics Space Physics Research 
\newcommand{\bain}{Bull.~Astron.~Inst.~Netherlands}% 
          % Bulletin Astronomical Institute of the Netherlands 
\newcommand{\fcp}{Fund.~Cosmic~Phys.}% 
          % Fundamental Cosmic Physics 
\newcommand{\gca}{Geochim.~Cosmochim.~Acta}% 
          % Geochimica Cosmochimica Acta 
\newcommand{\grl}{Geophys.~Res.~Lett.}% 
          % Geophysics Research Letters 
\newcommand{\jcp}{J.~Chem.~Phys.}% 
          % Journal of Chemical Physics 
\newcommand{\jgr}{J.~Geophys.~Res.}% 
          % Journal of Geophysics Research 
\newcommand{\jqsrt}{J.~Quant.~Spec.~Radiat.~Transf.}% 
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer 
\newcommand{\memsai}{Mem.~Soc.~Astron.~Italiana}% 
          % Mem. Societa Astronomica Italiana 
\newcommand{\nphysa}{Nucl.~Phys.~A}% 
          % Nuclear Physics A 
\newcommand{\physrep}{Phys.~Rep.}% 
          % Physics Reports 
\newcommand{\physscr}{Phys.~Scr}% 
          % Physica Scripta 
\newcommand{\planss}{Planet.~Space~Sci.}% 
          % Planetary Space Science 
\newcommand{\procspie}{Proc.~SPIE}% 
          % Proceedings of the SPIE 
\endinput
